A Fast, 2D Gaussian Process Method Based on Celerite: Applications to Transiting Exoplanet Discovery and Characterization

Gaussian processes (GPs) are commonly used as a model of stochastic variability in astrophysical time series. In particular, GPs are frequently employed to account for correlated stellar variability in planetary transit light curves. The efficient application of GPs to light curves containing thousands to tens of thousands of datapoints has been made possible by recent advances in GP methods, including the celerite method. Here we present an extension of the celerite method to two input dimensions, where, typically, the second dimension is small. This method scales linearly with the total number of datapoints when the noise in each large dimension is proportional to the same celerite kernel and only the amplitude of the correlated noise varies in the second dimension. We demonstrate the application of this method to the problem of measuring precise transit parameters from multiwavelength light curves and show that it has the potential to improve transit parameters measurements by orders of magnitude. Applications of this method include transit spectroscopy and exomoon detection, as well a broader set of astronomical problems.

==> section4.tex <==
\section{The \celerite Method in One and Two Dimensions}\label{sec:celerite}

    \subsection{The \celerite method}

        Until recently, adoption of GP methods has been limited by 
        computational expense. As a reminder, the log-likelihood function for a GP 
        model for a series of $N$ flux measurements 
        $\bvec{y}=(y_1, y_2, \dots y_N)$ taken at times 
        $\bvec{t} = (t_1, t_2, \dots t_N)$ is given by 
        \begin{equation}
	        \label{eqn:simple_logL_v2}
		    \ln\ \mathcal{L} = 
		    -\frac{1}{2}(\bvec{y}-\bvec{\mu})^\T K^{-1}(\bvec{y}-\bvec{\mu})  
		    -\frac{1}{2}\ln\ \mathrm{det}(K) - \frac{N}{2}\ln(2\pi)
	    \end{equation}
	    where $\bvec{\mu} = (\mu(t_1), \mu(t_2), \dots \mu(t_N))$ and 
	    $K$ is the covariance matrix of the GP. This equation involves 
	    the inverse and determinant of the $N\times N$ matrix $K$. In general, computing 
	    the inverse and determinant of an $N\times N$ matrix requires $\mathcal{O}(N^3)$ 
	    operations. Thus computing the likelihood for a GP by directly 
	    inverting $K$ becomes prohibitively expensive for datasets larger 
	    than about $10^4$ observations \citep{Deisenroth2015}. This is especially true for 
	    applications that require repeated calls to the likelihood function 
	    as is the case for minimization and MCMC. 
	
	    The computational expense of GPs can be mitigated in two ways. 
        The first is by employing inexact methods in which the 
        full GP covariance matrix is approximated by a matrix for 
        which the relevant matrix operations (primarily inversion 
        and computation of the determinant) can be computed more 
        efficiently than $\mathcal{O}(N^3)$ \citep{Rasmussen2006}. 
        The second is by restricting 
        the user to covariance matrices of a specific form for which, 
        again, the relevant matrix operations are quicker to compute; 
        \celerite \citep{Foreman-Mackey2017} is a member of this 
        second class of methods. \celerite is a fast,     
        one-dimensional 
        GP method which takes $\mathcal{O}(NJ^2)$ operations to 
        compute where $J$ is the number of \celerite terms that make 
        up the kernel function. For commonly-used kernel models the number of 
        terms will be very small compared to $N$. 
        
        \celerite works by representing the GP covariance matrix 
        as the sum of a diagonal matrix and $J$ semi-separable matrices. The Cholesky 
        factorization of $J$ semi-separable matrices plus a diagonal matrix 
        can be computed in $\mathcal{O}(NJ^2)$ rather than 
        the $\mathcal{O}(N^3/3)$ required for an ordinary 
        matrix. Once the Cholesky factors are in hand, the 
        inverse and determinant of the covariance matrix 
	    can be computed in $\mathcal{O}(NJ)$ and $\mathcal{O}(N)$ 
	    respectively. Here we briefly describe the 
	    \celerite algorithm, referring the reader to 
	    \citet{Foreman-Mackey2017} for a more detailed exposition of the method. 
		
		Consider a one-dimensional Gaussian process evaluated at the coordinates
		\begin{equation}
			\bvec{x} = \expandvec{t_1}{t_N}
		\end{equation}
		The \celerite kernel is given by
		\begin{eqnarray}
		    \label{eqn:k_alpha}
			k_\bvec{\alpha}(t_n, t_m) &=& \sigma_n^2 \delta_{nm} + \sum_{j=1}^J 
			% Re\left[(a_j+ib_j) e^{-(c_j+id_j)\tau_{nm}} + (a_j-ib_j)e^{(c_j-id_j)\tau_{nm}}\right] % This differs by a factor of 2 from the celerite paper
			\frac{1}{2}\left[(a_j+ib_j) e^{-(c_j+id_j)\tau_{nm}} \right. \cr &+& \left.  (a_j-ib_j)e^{(c_j-id_j)\tau_{nm}}\right]   % This fine
			%Re\left[(a_j+ib_j) e^{-(c_j+id_j)\tau_{nm}} + )\right]  % This is also fine
		\end{eqnarray}
		where $\bvec{\alpha} = (a_1...a_j, b_1...b_j, c_1...c_j, d_1...d_j)$, $\sigma_n^2$ is the variance of the Gaussian-distributed white noise, and $\tau_{nm} = |t_n-t_m|$. 
		This kernel defines a \celerite model with $J$ terms. 
		
		For a kernel function of this form, the covariance matrix is a symmetric, semiseparable matrix with semiseparability rank $R=2J$. A matrix of this type can 
		be written in terms of two generator matrices $U$ and $V$, both of size $(N\times 2J)$, along with a diagonal matrix $A$:
		\begin{equation}
		\label{eqn:KUV}
			K = A + \mathrm{tril}(UV^\T) + \mathrm{triu}(VU^\T),
		\end{equation}	
		where tril is the lower-triangular operator which, when applied to 
		a square matrix, preserves the entries below the diagonal and 
		replaces all entries on and above the diagonal with zeros. The triu operator 
		does the same for the upper-triangular entries in the matrix.
		In the case of our covariance matrix, the generator matrices are specified by:	
		\begin{eqnarray}
		    \label{eqn:UV_defs}
			U_{n, 2j-1} &=& a_je^{-c_jt_n}\cos(d_jt_n) + b_je^{-c_jt_n}\sin(d_jt_n), \cr
			U_{n, 2j} &=& a_je^{-c_jt_n}\sin(d_jt_n) - b_je^{-c_jt_n}\cos(d_jt_n), \cr
			V_{m, 2j-1} &=& e^{c_jt_m}\cos(d_jt_m), \cr
			V_{m, 2j} &=& e^{c_jt_m}\sin(d_jt_m),
		\end{eqnarray}
		and A is given by:
		\begin{equation}
		    \label{eqn:A_matrix}
			A_{n,n} = \sigma_n^2 + \sum_{j=1}^Ja_j.
		\end{equation}
		Computing the Cholesky decomposition for this covariance matrix can be accomplished in $\mathcal{O}(NJ^2)$ operations, allowing for the 
		fast computation of the GP likelihood function\footnote{The algorithm is described in \S \ref{sec:cholesky}}. 
		
		The kernel function implemented by \celerite is versatile in that 
	    by choosing appropriate coefficients it can be made to approximate a 
	    wide range of other kernel functions. This versatility is demonstrated in 
	    Fig.\ \ref{fig:approx_kerns} which shows approximations of several popular 
	    kernels achieved by carefully choosing $\left\{a_j\right\}$, $\left\{b_j\right\}$, $\left\{c_j\right\}$ and $\left\{d_j\right\}$. 
		Since each of these kernels may be approximated well by a \celerite kernel,
		the products and sums of these component kernels are also \celerite kernels, meaning that
		complex kernels can still be approximated within the \celerite kernel formalism.
		
		\begin{figure}
		    \centering
		    \includegraphics[width=\hsize]{plots/kernel_approx.png}
		    \caption{Approximation to various commonly used GP kernels %using the \celerite kernel.
		    (a) Simple kernels with an exact \celerite representation: %constant, exponential,
		    cosine, or exponential times cosine. (b) Approximation of a %Gaussian kernel (typically
		    referred to as ``exponential-squared" to distinguish it from %the GP). (c) Exponential
		    sine-squared kernels. (d) Matern kernels.}
		    \label{fig:approx_kerns}
		\end{figure}
        
    \subsection{Two-dimensional celerite method}
    \label{sec:2dcelerite}
        The version of \celerite outlined above is an inherently one-dimensional GP method. 
        While this is sufficient for many problems, such as modeling monochromatic light curves, 
        there are many other cases where we need to model covariance in two or more dimensions. 
        Here we describe two methods for 
        computing 2D Gaussian processes that 
        take advantage of the favorable scaling 
        of the one-dimensional \texttt{celerite} 
        method. The first applies when the 
        covariance matrix in the second dimension 
        can be written as the outer product 
        of a vector with itself. This applies 
        to the common task of modeling time-variable 
        spectra. The second, more general, method 
        has a less favorable scaling but allows 
        for the computation of GPs with an 
        arbitrary covariance matrix in the 
        second dimension. 
        
        \subsection{Overview}
            Consider the coordinate space $T\times U$ defined by the two vectors:
            \begin{eqnarray}
                \label{eqn:vec_defs}
                \bvec{t} &= \expandvec{t_1}{t_N} \\
	            \bvec{u} &= \expandvec{u_1}{u_M}
            \end{eqnarray}
            We can represent these coordinates in the form of an $N\times M$ 
            coordinate matrix $X$: 
            \begin{equation}
                X = \begin{bmatrix}
                    (t_1, u_1) & \hdots & (t_1, u_M) \\
                    \vdots &  \ddots & \\
                    (t_N, u_1) & & (t_N, u_M)
                \end{bmatrix}
            \end{equation}
            such that $X_{n, m} = (t_n, u_m)$. These coordinates correspond 
            to a matrix of observations at each coordinate which we call $Y$, where
            the entry $Y_{n, m}$ corresponds to the observation made at coordinate 
            $X_{n, m} = (t_n, u_m)$. In the discussion that follows we will 
            occasionally make use of the $\mathrm{vec}$ operator, which transforms 
            a matrix into a vector consisting of the entries in the 
            matrix stacked row-wise. For instance, 
            \begin{equation}
                \mvec{Y} = \left(y_{1, 1}, y_{1, 2}, ..., y_{1, M}, y_{2, 1}, y_{2, 2}, ..., y_{2, M}, ..., y_{N, M}\right)
            \end{equation}
            The shorthand $\bvec{x}$ and $\bvec{y}$ will be used to refer 
            to $\mvec{X}$ and $\mvec{Y}$ respectively. The mean of the GP, 
            $\mu_\bvec{\theta}$ will refer to a vector when taken as a function of 
            $\bvec{x}$ and as an $N\times M$ matrix when taken as a function 
            of $X$. 
            
            With these definitions the likelihood function 
            in the two-dimensional case is the same as 
            equation \ref{eqn:simple_logL}, with the 
            understanding that $\bvec{y}$ refers to 
            $\mathrm{vec}(Y)$, 
            $\bvec{\mu} = \mathrm{vec}(\mu(X))$, and 
            $K$ is a covariance matrix containing 
            pairwise covariance for each point 
            in our two-dimensional coordinate space.
            
            Consider the case where the covariance between 
            every pair of points on the grid 
            satisfies the equation 
            \begin{equation}
	            \label{eqn:multiplication_condition}
	    	    k(x_n, x_m) = \rho(t_i, t_j)\nu_{n,m}
	       \end{equation}
	       where $\rho$ is the kernel 
	       function describing the covariance 
	       in $t$, which depends on the 
	       separation between columns $i$ and $j$ of 
	       the coordinate matrix $X$, 
	       and $\nu_{n, m}$ is the covariance 
	       between rows $n$ and $m$ of $X$. 
	       If we assume no white noise 
	       (i.e. $k(x_n, x_n) = 0$), the covariance matrix 
	       may be written as a Kronecker product\footnote{
	            The Kronecker product between two matrices 
	            $A$ and $B$ with dimensions $n\times n$ and $p\times q$ respectively has 
	            dimensions $np\times mq$ and is given by the block matrix
	            \begin{equation}
	                A\otimes B = \begin{bmatrix}
                    a_{11}B & \dots & a_{1n}B \\
                    \vdots  & \ddots &\\
                    a_{n1}B & \dots  & a_{nn}B
                    \end{bmatrix}.
	            \end{equation}
	        } between the two one-dimensional covariance matrices for each 
	        of the coordinate directions in the grid. We write this Kronecker-structured 
	        covariance matrix as
	        \begin{equation}
	            \label{eqn:KTR}
	            K = T \otimes R
	        \end{equation}
	        where 
	        \begin{equation}
	            [T]_{i,j} = \rho(|t_i-t_j|)
	        \end{equation}
	        and $[R]_{n,m} = \nu_{n, m}$. We 
	        now discuss separately the decomposition 
	        of this covariance matrix when $R$ 
	        has the structure of an outer product 
	        as in equation \ref{eqn:R_outer} and 
	        the general case for arbitrarily 
	        defined $R$ matrices.
	        
	        \subsection{Outer product covariance 
	        matrices}
	        \label{sec:outer_product_method}
	        We start by writing $K$ in terms of the 
	        celerite generator matrices from 
	        equation \ref{eqn:KUV}:
	        \begin{eqnarray}
	            K &=& \Sigma + \left[A_0 + \mathrm{tril}(UV^\T) 
	            + \mathrm{triu}(VU^\T)\right] \otimes R \cr
	            &=& \Sigma + \mathrm{diag}(A_0\otimes R) \cr
	            &+& \mathrm{tril}(UV^\T\otimes R) 
	            + \mathrm{triu}(VU^\T\otimes R) 
	        \end{eqnarray}
	        where $A = \Sigma + A_0$ and $A_0$ is defined to 
	        be the white-noise free version of the $A$ matrix 
	        obtained by setting $\sigma_n = 0$ for all $n$. 
	        Substituting the outer product $\bvec{\alpha}\bvec{\alpha}^\T$ 
	        for $R$ inside the upper and lower triangular operators we 
	        have
	        \begin{eqnarray}
	            K = \Sigma &+& \mathrm{diag}(A_0\otimes R) \cr
	            &+& \mathrm{tril}(UV^\T\otimes \bvec{\alpha}\bvec{\alpha}^\T) \cr
	            &+& \mathrm{triu}(VU^\T\otimes \bvec{\alpha}\bvec{\alpha}^\T).
	        \end{eqnarray}
	        Applying the formula for mixed Kronecker and 
	        matrix products,
	        \begin{equation}
	            \label{eqn:mixed_products}
	            (AB)\otimes(CD) = (A\otimes C)(B\otimes D),
	        \end{equation}
	        we can rewrite the covariance matrix as 
	        \begin{eqnarray}
	            K = \Sigma &+& \mathrm{diag}(A_0\otimes R) \cr
	            &+& \mathrm{tril}((U\otimes \bvec{\alpha})(V\otimes \bvec{\alpha})^\T) \cr
	            &+& \mathrm{triu}((V\otimes \bvec{\alpha})(U\otimes \bvec{\alpha})^\T).
	        \end{eqnarray}
	        We now see that the two-dimensional covariance matrix 
	        has exactly the same semi-separable structure as 
	        the one-dimensional covariance matrix with new 
	        definitions of the generator matrices in terms of 
	        their Kronecker products with $\bvec{\alpha}$:
	        \begin{eqnarray}
	            \label{eqn:kronecker_generators_outer}
	            A' &=& \Sigma + \mathrm{diag}(A_0\otimes R) \cr
	            U' &=& U\otimes \bvec{\alpha} \\
	            V' &=& V\otimes \bvec{\alpha} \nonumber
	        \end{eqnarray}
	        Or, in terms of the \texttt{celerite} coefficients and 
	        the elements of $\bvec{\alpha}$:
	        \begin{eqnarray}
	            A'_{(p-1)n+p} &=& \Sigma_{(p-1)n+p} + \alpha_p^2 A_n \cr
	            U'_{(p-1)n+p, 2j-1} &=& \alpha_p U_{n, 2j-1} \cr
	            U'_{(p-1)n+p, 2j} &=& \alpha_p U_{n, 2j} \\
	            V'_{(p-1)n+p, 2j-1} &=& \alpha_p V_{n, 2j-1} \cr
	            V'_{(p-1)n+p, 2j} &=& \alpha_p V_{n, 2j} \nonumber
	        \end{eqnarray}
	        where the elements of $U$, $V$, and $A$ are defined in 
	        equation \ref{eqn:UV_defs} and $p$ ranges over $(1, M)$ 
	        with $M$ the length of the vector $\bvec{\alpha}$.
	        
	        \subsection{Arbitrary covariance matrices}
	        \label{sec:arbitrary_covariance_method}
	        In this section we assume that the covariance in 
	        $\bvec{u}$, defined by the covariance matrix 
	        $R$ is arbitrary, subject to 
	        the constraint that the full covariance matrix $K$ 
	        must be positive definite \footnote{Positive definiteness 
	        can be defined by the requirement that all eigenvalues 
	        of the matrix are positive. For a 1D 
	        \celerite model positive definiteness can be guaranteed 
	        by the methods outlined in Appendix A of \cite{Foreman-Mackey2017}. For a 2D \celerite model 
	        guaranteeing positive definiteness is more complicated, and 
	        we recommend investigating kernels on a case-by-case basis.}. 
	        
	        We again start by rewriting $T$ in terms of the 
	        celerite generator matrices $A$, $U$, and $V$ 
	        from equation \ref{eqn:KUV}:
	        \begin{eqnarray}
	            K &=& \Sigma + \left[A_0 + \mathrm{tril}(UV^\T) 
	            + \mathrm{triu}(VU^\T)\right] \otimes R \cr
	            &=& \Sigma + \mathrm{diag}(A_0\otimes R) \cr
	            &+& \mathrm{tril}(UV^\T\otimes R) 
	            + \mathrm{triu}(VU^\T\otimes R) 
	        \end{eqnarray}
	        We rewrite $R$ as $R I_M$ where $I_M$ is the $M\times M$ 
	        identity matrix, which allows us to write $K$ as 
	        \begin{eqnarray}
	            K = \Sigma &+& \mathrm{diag}(A_0\otimes R) \cr
	            &+& \mathrm{tril}((U\otimes R)(V\otimes I_M)^\T) \\
	            &+& \mathrm{triu}((V\otimes I_M)(U\otimes R)^\T) \nonumber 
	        \end{eqnarray}
	        where we have again applied equation \ref{eqn:mixed_products}. 
	        As for the outer product case, we now have a semi-separable 
	        matrix defined by a new set of generators: 
	        \begin{eqnarray}
	            \label{eqn:kronecker_generators}
	    	    \nonumber A' &=& \Sigma + \mathrm{diag}(A_0\otimes T) \\
    		    \nonumber U' &=& U\otimes T \\
	    	    V' &=& V\otimes I_M.
	        \end{eqnarray}
	        In terms of the \texttt{celerite} coefficients the 
	        generator matrices are defined element-wise as follows:
	        \begin{eqnarray}
    	    \label{eqn:UV_prime_defs}
    	        A'_{(n-1)M+p, (n-1)M+p} &=& \sigma_{(n-1)M+1}^2 + R_{p, p}\sum_{j=1}^J a_j \cr
    	        U'_{(n-1)M+p,(2j-1)M+q} &=& R_{p, q}U_{n, 2j-1} \\
    	        U'_{(n-1)M+p, 2jM+q} &=& R_{p, q}U_{n, 2j} \cr
    	        V'_{(n-1)M+p,(2j-1)M+q} &=& \delta_{p, q}V_{n, 2j-1} \cr
    	        V'_{(n-1)M+p, 2jM+q} &=& \delta_{p, q}V_{n, 2j}, \nonumber
        	\end{eqnarray}
        	where $p$ and $q$ range over $(1, M)$ and $\delta_{p, q}$ is the 
        	Kronecker delta function:
        	\begin{equation}
    	        \delta_{p, q} = \left\{\begin{matrix}
    	            1 & p=q \\
    	            0 & p\neq q
    	        \end{matrix}\right.
	        \end{equation}
	        At this point we can apply the \celerite algorithms 
    	    to this new set of generator matrices with only 
    	    a few minor alterations. The 
    	    algorithms for factorizing the matrix, sampling from the GP, and 
    	    computing the likelihood are given in the following sections. The 
    	    algorithm for GP prediction/interpolation are described in appendix \ref{sec:prediction}.
    	    
    	\subsection{Cholesky Factorization} \label{sec:cholesky}
    	
    	We begin by introducing the Cholesky factorization 
    	algorithm for the one-dimensional method 
    	as given in \cite{Foreman-Mackey2017}. The Cholesky factorization 
    	of the covariance matrix $K$ is given by 
    	\begin{equation}
    	    K = LDL^\T
    	\end{equation}
    	where $L$ is the lower-triangular Cholesky factor and 
    	$D$ is a diagonal matrix. Our task is to find 
    	the matrices $L$ and $D$. The starting point for the 
    	\texttt{celerite} algorithm is the ansatz that 
    	the Cholesky factor has the form 
    	\begin{equation}
    	    L = I + \mathrm{tril}(UW^\T)
    	\end{equation}
    	where $U$ is the generator matrix that we're already 
    	familiar with and $W$ is an unknown matrix of 
    	the same dimensions as $U$. $W$ and $D$ can then 
    	be found via the recursion relations
    	\begin{eqnarray}
    	     \nonumber S_{n, j, k} = S_{n-1, j, k} + D_{n-1, n-1}W_{n-1, j}W_{n-1, k} \\
    	    \nonumber D_{n, n} = A_{n, n} - \sum_{j=1}^R\sum_{k=1}^RU_{n,j}S_{n, j, k}U_{n, k} \\
    	    W_{n, j} = \frac{1}{D_{n, n}}\left[V_{n, j} - \sum_{k=1}^RU_{n, k}S_{n, j, k}\right],
    	\end{eqnarray}
    	where $S_{1, j, k}$ is a matrix of zeros. In the original 
    	\texttt{celerite} paper it was found that, in order to 
    	avoid numerical stability issues caused by the 
    	exponential factors in equation \ref{eqn:UV_defs}, it was 
    	necessary to redefine the generator matrices $U$ and $V$ 
    	and to define an additional matrix $\phi$ of the same 
    	dimensions as $U$ and $V$. The generators become
    	\begin{eqnarray}
    	    \tilde U_{n, 2j-1} &=& a_j\cos(d_jt_n) + b_j\sin(d_jt_n) \cr 
			\tilde U_{n, 2j} &=& a_j\sin(d_jt_n) - b_j\cos(d_jt_n) \cr
			\tilde V_{m, 2j-1} &=& \cos(d_jt_m) \\
			\tilde V_{m, 2j} &=& \sin(d_jt_m). \nonumber
		\end{eqnarray}
		The unknown matrix $W$ becomes 
		\begin{eqnarray}
			\tilde W_{n, 2j-1} &=& e^{-c_jt_n}W_{n, 2j-1} \cr
			\tilde W_{n, 2j} &=& e^{-c_jt_n}W_{n, 2j}.
    	\end{eqnarray}
    	And the new matrix $\phi$ is defined
    	\begin{eqnarray}
    	    \phi_{n, 2j-1} = \phi_{n, 2j} = e^{-c_j(t_n-t_{n-1})}.
    	\end{eqnarray}
    	The algorithm for decomposing the covariance matrix 
    	becomes
    	\begin{eqnarray}
    	    \label{eqn:cholesky_algorithm1}
    	    S_{n,j,k} &=& \phi_{n,j}\phi_{n,k}\left[S_{n-1, j, k} + D_{n-1, n-1}\tilde{W}_{n-1, j}\tilde{W}_{n-1,k}\right] \\
    	    D_{n, n} &=& A_{n, n} - \sum_{j=1}^{2J}\sum_{k=1}^{J2}\tilde U_{n, j}S_{n, j, k}\tilde U_{n, k} \\
    	    \label{eqn:cholesky_algorithm2}
    	    \tilde W_{n, j} &=& \frac{1}{D_{n, n}}\left[\tilde V_{n, j}-\sum_{k=1}^{2JM}\tilde U_{n, k}S_{n, j, k}\right].
    	\end{eqnarray}
    	
    	To decompose the covariance matrix for the two-dimensional 
    	GP we only need to make two changes. The first is to 
    	replace the generator matrices $U$ and $V$ with their 
    	Kronecker product counterparts $U'$ and $V'$, defined 
    	according to equations \ref{eqn:kronecker_generators_outer} or 
    	\ref{eqn:kronecker_generators}, and the second is to 
    	update the definition of $\phi$ to account for 
    	having multiple measurements taken at the same 
    	point in time (one for each gridpoint 
    	in the second dimension). 
    	
    	The recursive cholesky decomposition algorithm can be written 
    	in terms of $U'$ and $V'$ as:
    	\begin{eqnarray}
    	    \label{eqn:cholesky_algorithm_final}
    	    S_{n,j,k} &=& \phi'_{n,j}\phi'_{n,k}\left[S_{n-1, j, k} + D_{n-1, n-1}\tilde{W}_{n-1, j}\tilde{W}_{n-1,k}\right] \cr
    	    D_{n, n} &=& A'_{n, n} - \sum_{j=1}^{P}\sum_{k=1}^{P}\tilde U'_{n, j}S_{n, j, k}\tilde U'_{n, k} \\
    	    \tilde W_{n, j} &=& \frac{1}{D_{n, n}}\left[\tilde V'_{n, j}-\sum_{k=1}^{P}\tilde U'_{n, k}S_{n, j, k}\right] \nonumber
    	\end{eqnarray}
    	where $P$ is the number of rows in $U'$ and $V'$. For an 
    	outer-product covariance in the second dimension we 
    	have $P = 2J$, and for an arbitrary covariance 
    	we have $P = 2JM$ where $M$ is the length of the 
    	second dimension. $\phi'$ is the redefined $\phi$ matrix, 
    	with elements given by 
    	\begin{eqnarray}
    	    \phi'_{(p-1)n+p, :} = \left\{\begin{matrix}
    	        e^{-c_j(t_n-t_{n-1})} & p=1 \\
    	        1 & p > 1
    	    \end{matrix}\right. , 
    	\end{eqnarray}
    	with $p$ ranging over $(1, M)$ and the colon indicating 
    	that the element is identical for every entry of that 
    	row. The matrices $\tilde U'$ and $\tilde V'$ are 
    	simply the Kronecker product definitions of $U'$ and 
    	$V'$ from equations \ref{eqn:kronecker_generators_outer} 
    	and \ref{eqn:kronecker_generators} taken with $\tilde U$ 
    	and $\tilde V$ rather than $U$ and $V$. 
    	
    	The recursive algorithm defined above 
    	requires one pass through each of the $NM$ rows 
    	of $\tilde U'$ and $\tilde V'$. At each step we 
    	compute a double sum over the $P$ columns of these matrices. 
    	The resultant scaling is thus $\mathcal{O}(NMP^2)$. When 
        the covariance matrix for the second dimension, $R$ is 
        an outer product we have $P=2J$ and the method scales 
        as $\mathcal{O}(NMJ^2)$. This is the most favorable case. 
        In the case that $R$ is an arbitrary covariance matrix 
        of size $M\times M$, we obtain the scaling $\mathcal{O}(NJ^2M^3)$ 
        since $P=2JM$. 
    	
    	% everything below may need changed. consider removing 
    	% details of algorithms besides prediction.  Also remove 
    	% 'proof' section of appendix. I don't think it's necessary 
    	% anymore.

    	\subsection{Drawing a sample from the GP}
    	The procedure for drawing a sample from the GP is unaltered from 
    	the one-dimensional algorithm except for the replacement of the 
    	un-primed matrices with the Kronecker-structured primed matrices. 
    	To draw a sample from the GP is to compute 
    	\begin{equation}
    	    \bvec{y} = \bvec{\mu_\theta}(\bvec{z}) + L\bvec{z},
    	\end{equation}
    	where $L$ is the lower triangular Cholesky factor of $K$ 
    	and \bvec{z} is a vector of values drawn from the unit normal distribution 
    	$z_i \sim \mathcal{N}(0, 1)$. The algorithm is given by
    	\begin{eqnarray}
    	    f_{n, j} &=& \phi_{n, j}\left[f_{n-1, j} + \tilde W_{n-1, j}\sqrt{D_{n-1, b-1}z_{n-1}}\right] \\
    	    y_n &=& D_{n, n}z_n + \sum_{j=1}^{P}\tilde U'_{n, j}f_{n, j}.
    	\end{eqnarray}
    	In order to visualize the sample we've drawn we will need to unpack the 
    	vector $\bvec{y}$ into $M$ separate vectors, one for each point 
    	$\bvec{u}=\expandvec{u_1, u_2}{u_M}$, each containing the sample 
    	evaluated at the points $\bvec{t}=\expandvec{t_1, t_2}{t_N}$. If 
    	$\bvec{t}$ is indexed by $i$ and $\bvec{u}$ is indexed by $j$, then 
    	the sample evaluated at point $(t_i, u_j)$ is given by $y_{M(i-1)+j}$.
    	
    	This algorithm requires one pass through the $NM$ rows of 
    	$\tilde W$ and $\tilde U'$, and a single pass through the 
    	$P$ columns of $\tilde U'$, and therefore scales as $\mathcal{O}(NMJ)$ in the case that $R$ can be written 
    	as an outer product and $\mathcal{O}(NJM^2)$ for 
    	arbitrarily defined $R$. 
    	Figures \ref{fig:sho_psd}, \ref{fig:comparison}, 
    	and \ref{fig:regimes} show examples of GP samples.
    	
    	\subsection{Computing the likelihood}
    	\label{sec:likelihood}
    	The likelihood, given in equation \ref{eqn:simple_logL}, incorporates 
    	the inverse and log-determinant of $K$. We therefore first 
    	describe the algorithms for each of these computations. For \celerite 
    	models we can compute products of the inverse covariance matrix with 
    	a vector, $\bvec{z} = K\bvec{y}$ using a two-part algorithm. 
    	We first compute the intermediary $\bvec{z}'$
    	\begin{eqnarray}
    	    \label{eqn:inv1}
    	    f_{n,j} &=& \phi_{n,j}\left[f_{n-1, j}+\tilde W_{n-1, j}z'_{n-1}\right] \\
    	    z'_{n} &=& y_n - \sum_{j=1}^{P}\tilde U'_{n, j}f_{n,j}
    	\end{eqnarray}
    	which we then use to compute $\bvec{z}$ in the second step of the algorithm 
    	\begin{eqnarray}
    	    g_{n,j} &=& \phi_{n+1,j}\left[g_{n+1, j} + \tilde U'_{n+1, j}z_{n+1}\right] \\
    	    \label{eqn:inv2}
    	    z_n &=& \frac{z'_n}{D_{n,n}} - \sum_{j=1}^{P}\tilde W_{n,j}g_{n,j}
    	\end{eqnarray}
    	where $g_{N+1, j} = 0$ for all $j$. The log-determinant of $K$ is 
    	given by 
    	\begin{equation}
    	    \ln{(\det K)} = \sum_{n=1}^{N}\ln{(D_{n,n})}
    	\end{equation}
    	Putting these two steps together we can compute the 
    	log-likelihood 
    	for the \celerite model. Because the algorithm for taking products of the 
    	inverse requires $\mathcal{O}(NMP)$ operations, whereas the log-determinant 
    	can be computed in only $\mathcal{O}(NM)$ operations, the log-likelihood 
    	computation as a whole scales as $\mathcal{O}(NMP)$.
    	In practice, the 
    	bottleneck for applications such as maximizing the likelihood or MCMC 
    	is computing the Cholesky factor rather than computing the log-likelihood, 
    	since the log-likelihood computation itself 
    	is faster by $\mathcal{O}(JM)$. Figure 
    	\ref{fig:benchmarks} shows benchmarks for the Cholesky factorization 
    	computation as a function of the size of each relevant dimension for the 
    	problem, separately for 
    	arbitrary and outer-product definitions of $R$.
    	
    	\subsection{Predicting and Extrapolating}
    	A Gaussian process prediction is an interpolation 
    	of observed data with a GP model. Extrapolation 
    	is mathematically equivalent to prediction but 
    	an extrapolation is computed beyond the observation 
    	coordinates or grid.  ``Prediction'' can also be carried out at the observed locations, which consists of an estimate of the data with white noise removed (this amounts to a filter which is customized to the power-spectrum of the GP kernel).
    	
    	\begin{figure*}[t]
	        \plotone{plots/prediction.png}
            \caption{A demonstration of GP prediction. \textbf{Left:} A realization 
            of a 2D GP noise model with heteroskedastic white noise. The 
            black lines are a GP prediction for a GP with the same parameters for 
            which the realization was computed.
            \textbf{Right:} Residuals showing that the correlated variability 
            is correctly modeled by the GP. Once the prediction has been subtracted from 
            the simulated observations  
            we are left with only the estimated 
            white noise component.}
            \label{fig:prediction}
        \end{figure*}
    	
    	The predictive distribution of a Gaussian process is 
    	a multivariate normal with a mean $\mu^*$ and covariance $K^*$ evaluated at 
    	the input coordinates $\bvec{x}^*$. For a 
    	GP with no white noise component the mean is constrained 
    	to pass directly through each observation of the data 
    	points $\bvec{y}$. For a GP with a non-zero white noise 
    	component the GP will act as a filter such that when the mean 
    	is subtracted from the data the residuals will be distributed 
    	according to 
    	a Gaussian distribution whose width is given by the 
    	GP white noise. Figure \ref{fig:prediction} demonstrates 
    	this for simulated 2D noise. On the left is a simulated 
    	dataset containing correlated and white noise. The white 
    	noise is heteroskedastic (varying in amplitude) with respect 
    	to both dimensions. The right panel shows the residuals 
    	when a GP trained on the data in the left panel is used 
    	as a filter to remove correlated noise. 
    	
    	The predictive mean and covariance is computed as follows 
    	\begin{eqnarray}
    	\label{eqn:predictive_mean}
    	    \bvec{\mu^*} &=& \bvec{\mu_\theta}(\bvec{x^*}) + K(\bvec{x^*}, \bvec{x})K(\bvec{x}, \bvec{x})^{-1}[\bvec{y}-\bvec{\mu_\theta}(\bvec{x})] \\
    	    K^* &=& K(\bvec{x^*}, \bvec{x^*}) - K(\bvec{x^*}, \bvec{x})K(\bvec{x}, \bvec{x})^{-1}K(\bvec{x}, \bvec{x^*})
    	\end{eqnarray}
    	where $K(\bvec{x^*}, \bvec{x})$ and $K(\bvec{x}, \bvec{x^*})$ are the covariance 
    	kernel evaluated between the input coordinates and the data coordinates. If 
    	the input coordinates consist of $P$ points in the first dimension and 
    	$S$ points in the second then these matrices have dimensions $(PS\times NM)$ 
    	and $(NM\times PS)$ respectively. 
    	
    	For the 2D Kronecker-structured covariance matrix 
    	$K = T\otimes R$, we can rewrite equation \ref{eqn:predictive_mean} 
    	as 
    	\begin{eqnarray}
    	    \label{eqn:prediction_kron}
    	    \bvec{\mu}^* &=& \bvec{\mu_\theta}(\bvec{x}^*) + \left[T(\bvec{x}^*, \bvec{x})\otimes R(\bvec{x}^*, \bvec{x})\right]K(\bvec{x}, \bvec{x})^{-1}[\bvec{y}-\bvec{\mu}_\bvec{\theta}(\bvec{x})] \\
    	    &=& \bvec{\mu_\theta}(\bvec{x}^*) + \left[T(\bvec{x}^*, \bvec{x})\otimes R(\bvec{x}^*, \bvec{x})\right]\bvec{z}
    	\end{eqnarray}
    	where $\bvec{z} = K(\bvec{x}, \bvec{x})^{-1}\left[\bvec{y}-\bvec{\mu}_\bvec{\theta}(x)\right]$
    	Writing the second term of equation \ref{eqn:prediction_vec} in terms 
    	of the vectorization operator we have
    	\begin{equation}
    	    \label{eqn:prediction_vec}
    	    \left[T(\bvec{x}^*, \bvec{x})\otimes R(\bvec{x}^*, \bvec{x})\right]\bvec{z}
    	     = \left[T(\bvec{x}^*, \bvec{x})\otimes R(\bvec{x}^*, \bvec{x})\right]\mvec{Z}
    	\end{equation}
    	where $Z = Y - \mu_\theta(X)$. For matrices $A$, $B$, and $C$ of sizes $(n\times m)$, $(m, p)$, and $(p, q)$ 
    	respectively there is an identity that 
    	states the following: 
    	\begin{equation}
    	    \mvec{ABC} = (A\otimes C^\T)\mvec{B}.
    	\end{equation} Applying this to 
    	equation \ref{eqn:prediction_vec} gives 
    	\begin{equation}
    	    \left[T(\bvec{x}^*, \bvec{x})\otimes R(\bvec{x}^*, \bvec{x})\right]\bvec{z} = \mvec{TZR}.
    	\end{equation}
    	The full expression for the predictive mean is now 
    	\begin{equation}
    	    \bvec{\mu}^* = \bvec{\mu}_\bvec{\theta}(\bvec{x}^*) + \mvec{TZR}.
    	\end{equation} 
    	
    	The matrix product $TZR$ can be computed via a modified version of 
    	the \celerite prediction algorithm presented in \citep{Foreman-Mackey2017}.
    	In essence, for each pass through the loop used to compute the prediction 
    	in the one-dimensional case, we first need to compute the entries in one 
    	column of $ZR$, at an additional expense of $M^2$. The algorithm therefore 
    	requires $\mathcal{O}(nNM^2 + pPM^2)$ operations, where 
    	$n$ and $p$ are constant factors. The full 2D 
    	prediction algorithm is presented in appendix \ref{sec:prediction}. 

	    \begin{figure*}[t]
	        \plottwo{plots/benchmarks_NM.pdf}{plots/benchmarks_NJ.pdf}
	        \plottwo{plots/benchmarks_MN.pdf}{plots/benchmarks_MJ.pdf}
	        \plottwo{plots/benchmarks_JN.pdf}{plots/benchmarks_JM.pdf}
            \caption{Benchmarks for our 2D celerite implementation. The first 
            two panels show the scaling of computation time with the number of points in 
            the first dimension, which is $\mathcal{O}(N)$. The second two panels show 
            the scaling of computation time with the number of points in the second 
            dimension, which is $\mathcal{O}(M^3)$ since the algorithm does not benefit from 
            the properties of a semiseparable covariance matrix in this direction. The final 
            two panels show the scaling with the number of terms, $J$, which is $\mathcal{O}(J^2)$}. 
            \label{fig:benchmarks}
        \end{figure*}
        
        This completes our description of our two-dimensional extension of the \celerite algorithm.  We now return to our results from above and discuss their implications.
    
